Relaxation Labeling Meets GANs: Solving Jigsaw Puzzles with Missing Borders

This paper proposes JiGAN, a GAN-based method for solving Jigsaw puzzles with eroded or missing borders. Missing borders is a common real-world situation, for example, when dealing with the reconstruction of broken artifacts or ruined frescoes. In this particular condition, the puzzle's pieces do not align perfectly due to the borders' gaps; in this situation, the patches' direct match is unfeasible due to the lack of color and line continuations. JiGAN, is a two-steps procedure that tackles this issue: first, we repair the eroded borders with a GAN-based image extension model and measure the alignment affinity between pieces; then, we solve the puzzle with the relaxation labeling algorithm to enforce consistency in pieces positioning, hence, reconstructing the puzzle. We test the method on a large dataset of small puzzles and on three commonly used benchmark datasets to demonstrate the feasibility of the proposed approach.

==> tables_benchmark.tex <==
\begin{table}[t!]
\parbox{.45\linewidth}{
\caption{Benchmark datasets. RL with and without GAN. Direct accuracy}
\label{tab:table3}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Direct } & \textit{no gap} & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
                            & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
                            \hline
\textit{70 pieces}  & 0.97      & 0.22          & \textbf{0.51}            & 0.11          & \textbf{0.32}           \\
\textit{88  pieces}  & 0.99      & 0.23         & \textbf{0.59}            & 0.07          & \textbf{0.31}           \\
\textit{150 pieces} & 0.99      & 0.12          & \textbf{0.38}            & 0.06          & \textbf{0.15}           \\
\hline
 mean                           & \textbf{0.98}       & 0.19 & \textbf{0.49}   & 0.08 & \textbf{0.26}  
\end{tabular}}
}
\hfill
\parbox{.45\linewidth}{

\caption{Benchmark datasets. RL with and without GAN. Neighbour accuracy}
\label{tab:table4}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Neighbour } & \textit{no gap} & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
                            & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
                            \hline
\textit{70  pieces }  & 0.97      & 0.46          & \textbf{0.66}            & 0.35          & \textbf{0.45}            \\
\textit{88  pieces}  & 0.99      & 0.46          & \textbf{0.65}            & 0.30          & \textbf{0.40}            \\
\textit{150 pieces} & 0.99      & 0.41          & \textbf{0.54}            & 0.28          & \textbf{0.33}            \\
\hline
  mean                          & \textbf{0.98}      & 0.45 & \textbf{0.62}   & 0.31 & \textbf{0.39}  
\end{tabular}}
}
\end{table}

==> tables_pacs.tex <==
\begin{table}[t!]
\parbox{.45\linewidth}{
\caption{PACS dataset. RL vs. \name, Direct accuracy}
\label{tab:table1}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Direct acc.}                & \textit{no gap}    & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
\textbf{} & \textbf{RL} & \textbf{RL}      & \textbf{\name}  & \textbf{RL}       & \textbf{\name}   \\
\hline
\textit{house}    & 0.92 & 0.57 & \textbf{0.74} & 0.41 & \textbf{0.60} \\
\textit{elephant} & 0.88 & 0.51 & \textbf{0.74} & 0.30 & \textbf{0.54} \\
\textit{guitar}   & 0.83 & 0.42 & \textbf{0.65} & 0.26 & \textbf{0.48} \\
\textit{person}   & 0.90 & 0.56 & \textbf{0.72} & 0.40 & \textbf{0.58} \\
\hline
   mean     & \textbf{0.88}      & 0.50    & \textbf{0.70}    & 0.32     & \textbf{0.53}\\
\end{tabular}}
}
\hfill
\parbox{.45\linewidth}{
\caption{PACS dataset.  RL vs. \name, Perfect ratio}
\label{tab:table2}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Perfect rec.}         & no gap & 7\% gap & 7\% gap & 14\% gap & 14\% gap \\
\textbf{} & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
\hline
\textit{house}    & 0.90   & 0.46    & \textbf{0.64}    & 0.26     & \textbf{0.42}     \\
\textit{elephant} & 0.86   & 0.41    & \textbf{0.64}    & 0.16     & \textbf{0.36}     \\
\textit{guitar}   & 0.77   & 0.33    & \textbf{0.49}    & 0.13     & \textbf{0.27}     \\
\textit{person}   & 0.89   & 0.51    & \textbf{0.65}    & 0.28     & \textbf{0.43}     \\
\hline
   mean                       & \textbf{0.85}      & 0.41 & \textbf{0.60}   & 0.19 & \textbf{0.35}  
\end{tabular}}
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[h!]
% \caption{PACS dataset. RL solver vs. \name, Direct accuracy}
% \label{tab:table1}
% \centering
% %\resizebox{0.45\textwidth}{!}{
% \begin{tabular}{l|c|cc|cc}
% \hline
% \textbf{Direct acc.}                & \textit{no gap}    & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
% \textbf{} & \textbf{RL} & \textbf{RL}      & \textbf{\name}  & \textbf{RL}       & \textbf{\name}   \\
% \hline
% \textit{house}    & 0.92 & 0.57 & \textbf{0.74} & 0.41 & \textbf{0.60} \\
% \textit{elephant} & 0.88 & 0.51 & \textbf{0.74} & 0.30 & \textbf{0.54} \\
% \textit{guitar}   & 0.83 & 0.42 & \textbf{0.65} & 0.26 & \textbf{0.48} \\
% \textit{person}   & 0.90 & 0.56 & \textbf{0.72} & 0.40 & \textbf{0.58} \\
% \hline
%         & \textbf{0.88}      & 0.50    & \textbf{0.70}    & 0.32     & \textbf{0.53}\\
% \end{tabular}%}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[h!]
% \caption{PACS dataset.  RL solver vs. \name, Perfect reconstruction ratio}
% \label{tab:table2}
% \centering
% \resizebox{0.45\textwidth}{!}{
% \begin{tabular}{l|c|cc|cc}
% \textbf{Perfect rec.}         & no gap & 7\% gap & 7\% gap & 14\% gap & 14\% gap \\
% \textbf{} & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
% \hline
% \textit{house}    & 0.90   & 0.46    & \textbf{0.64}    & 0.26     & \textbf{0.42}     \\
% \textit{elephant} & 0.86   & 0.41    & \textbf{0.64}    & 0.16     & \textbf{0.36}     \\
% \textit{guitar}   & 0.77   & 0.33    & \textbf{0.49}    & 0.13     & \textbf{0.27}     \\
% \textit{person}   & 0.89   & 0.51    & \textbf{0.65}    & 0.28     & \textbf{0.43}     \\
% \hline
%                           & \textbf{0.85}      & 0.41 & \textbf{0.60}   & 0.19 & \textbf{0.35}  
% \end{tabular}}
% \end{table}

==> tables_pacs_single.tex <==
\begin{table}[h!]
\caption{PACS dataset. RL solver vs. \name, Direct accuracy}
\label{tab:table1}
\centering
%\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\hline
\textbf{Direct acc.}                & \textit{no gap}    & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
\textbf{} & \textbf{RL} & \textbf{RL}      & \textbf{\name}  & \textbf{RL}       & \textbf{\name}   \\
\hline
\textit{house}    & 0.92 & 0.57 & \textbf{0.74} & 0.41 & \textbf{0.60} \\
\textit{elephant} & 0.88 & 0.51 & \textbf{0.74} & 0.30 & \textbf{0.54} \\
\textit{guitar}   & 0.83 & 0.42 & \textbf{0.65} & 0.26 & \textbf{0.48} \\
\textit{person}   & 0.90 & 0.56 & \textbf{0.72} & 0.40 & \textbf{0.58} \\
\hline
        & \textbf{0.88}      & 0.50    & \textbf{0.70}    & 0.32     & \textbf{0.53}\\
\end{tabular}%}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\caption{PACS dataset.  RL solver vs. \name, Perfect reconstruction ratio}
\label{tab:table2}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Perfect rec.}         & no gap & 7\% gap & 7\% gap & 14\% gap & 14\% gap \\
\textbf{} & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
\hline
\textit{house}    & 0.90   & 0.46    & \textbf{0.64}    & 0.26     & \textbf{0.42}     \\
\textit{elephant} & 0.86   & 0.41    & \textbf{0.64}    & 0.16     & \textbf{0.36}     \\
\textit{guitar}   & 0.77   & 0.33    & \textbf{0.49}    & 0.13     & \textbf{0.27}     \\
\textit{person}   & 0.89   & 0.51    & \textbf{0.65}    & 0.28     & \textbf{0.43}     \\
\hline
                          & \textbf{0.85}      & 0.41 & \textbf{0.60}   & 0.19 & \textbf{0.35}  
\end{tabular}}
\end{table}

==> tables_single.tex <==
\begin{table}[h!]
\caption{Benchmark datasets. RL with and without GAN. Direct accuracy}
\label{tab:table3}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Direct } & \textit{no gap} & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
                            & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
                            \hline
\textit{70 pieces}  & 0.97      & 0.22          & \textbf{0.51}            & 0.11          & \textbf{0.32}           \\
\textit{88  pieces}  & 0.99      & 0.23         & \textbf{0.59}            & 0.07          & \textbf{0.31}           \\
\textit{150 pieces} & 0.99      & 0.12          & \textbf{0.38}            & 0.06          & \textbf{0.15}           \\
\hline
                            & \textbf{0.98}       & 0.19 & \textbf{0.49}   & 0.08 & \textbf{0.26}  
\end{tabular}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\caption{Benchmark datasets. RL with and without GAN. Neighbour accuracy}
\label{tab:table4}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|c|cc|cc}
\textbf{Neighbour } & \textit{no gap} & \textit{7\% gap} & \textit{7\% gap} & \textit{14\% gap} & \textit{14\% gap} \\
                            & \textbf{RL} & \textbf{RL}   & \textbf{\name} & \textbf{RL}   & \textbf{\name} \\
                            \hline
\textit{70  pieces }  & 0.97      & 0.46          & \textbf{0.66}            & 0.35          & \textbf{0.45}            \\
\textit{88  pieces}  & 0.99      & 0.46          & \textbf{0.65}            & 0.30          & \textbf{0.40}            \\
\textit{150 pieces} & 0.99      & 0.41          & \textbf{0.54}            & 0.28          & \textbf{0.33}            \\
\hline
                            & \textbf{0.98}      & 0.45 & \textbf{0.62}   & 0.31 & \textbf{0.39}  
\end{tabular}}
\end{table}
